ReStyle3D: Scene-Level Appearance Transfer with Semantic Correspondences

We introduce ReStyle3D, a novel framework for scene-level appearance transfer from a single style image to a real-world scene represented by multiple views. The method combines explicit semantic correspondences with multi-view consistency to achieve precise and coherent stylization. Unlike conventional stylization methods that apply a reference style globally, ReStyle3D uses open-vocabulary segmentation to establish dense, instance-level correspondences between the style and real-world images. This ensures that each object is stylized with semantically matched textures. It first transfers the style to a single view using a training-free semantic-attention mechanism in a diffusion model. It then lifts the stylization to additional views via a learned warp-and-refine network guided by monocular depth and pixel-wise correspondences. Experiments show that ReStyle3D consistently outperforms prior methods in structure preservation, perceptual style similarity, and multi-view coherence. User studies further validate its ability to produce photo-realistic, semantically faithful results. Our code, pretrained models, and dataset will be publicly released, to support new applications in interior design, virtual staging, and 3D-consistent stylization.

==> figures/tex/qualitative_ablation.tex <==
\begin{figure*}[t]
\begin{center}
\centering
\includegraphics[width=0.85\linewidth]{figures/images/qualitative_ablation.pdf}
\end{center}
% \vspace{-15pt}
\caption{
% 
\textbf{Comparison between different auto-regression strategies.} The rows represent two non-sequential views used in multi-view appearance transfer, while the columns represent different frame selection strategies. (a) \textit{Single} warps only the previous view, failing to preserve details like the painting on the wall present in the top image, as pixel information is lost. (b) \textit{All} warps all past frames to the current frame, improving consistency but introducing smearing effects, demonstrated by the red arrows (highlighted by red arrows) due to overlapping pixel projections with large color value differences originating from lighting changes. (c) \textit{Ours}, the proposed strategy in \ours, achieves the most consistent and clean multi-view stylization.
}
% \vspace{-15pt}
\label{fig:ar_ablation}
\end{figure*}

\vspace{15pt}

\begin{figure*}[t]
\begin{center}
\centering
\includegraphics[width=0.99\linewidth]{figures/images/depth_condition.pdf}
\end{center}
% \vspace{-15pt}
\caption{
% 
\textbf{Qualitative comparison between two different conditional models.}  We train a warp-and-refine model without the monocular depth~(MDE) condition. Without MDE supervision, the model struggles to correct local alignment issues~(\eg, the door handle, wine bottles, and chairs), resulting in noticeable geometric distortions and texture artifacts. In contrast, incorporating MDE enables the model to leverage pixel-aligned depth cues and more faithfully reconstruct fine details, yielding sharper and more consistent multi-view results.
}
% \vspace{-15pt}
\label{fig:qualitative_ablation}
\end{figure*}

==> figures/tex/style_examples.tex <==
\begin{figure*}[t]
\begin{center}
\centering
\includegraphics[width=0.99\linewidth]{figures/images/style_examples.pdf}
\end{center}
% \vspace{-15pt}
\caption{
% 
\textbf{Style Image Samples. }We showcase exemplar images of various designs across various styles and types of rooms from our \dataset benchmark style image collection~(top rows), paired with their open-vocabulary semantic segmentation masks~(bottom rows). These images span a variety of interior spaces--including kitchens, living rooms, and bedrooms--and illustrate the core challenge of \ours: transferring the appearance of each semantically matched region~(e.g., cabinets, couches, and beds) from a style image to real-world 3D scenes. Our method leverages these semantic masks to ensure each object is stylized with the correct instance-level textures while maintaining photo-realism and multi-view consistency.
}
% \vspace{-15pt}
\label{fig:style_examples}
\end{figure*}
